Keyframe Demonstration Seeded and Bayesian Optimized Policy Search

This paper introduces a novel Learning from Demonstration framework to learn robotic skills with keyframe demonstrations using a Dynamic Bayesian Network (DBN) and a Bayesian Optimized Policy Search approach to improve the learned skills. DBN learns the robot motion, perceptual change in the object of interest (aka skill sub-goals) and the relation between them. The rewards are also learned from the perceptual part of the DBN. The policy search part is a semiblack box algorithm, which we call BO-PI2 . It utilizes the action-perception relation to focus the high-level exploration, uses Gaussian Processes to model the expected-return and performs Upper Confidence Bound type low-level exploration for sampling the rollouts. BO-PI2 is compared against a stateof-the-art method on three different skills in a real robot setting with expert and naive user demonstrations. The results show that our approach successfully focuses the exploration on the failed sub-goals and the addition of reward-predictive exploration outperforms the state-of-the-art approach on cumulative reward, skill success, and termination time metrics.

==> alg3.tex <==
\begin{algorithm}[H]
\caption{\onur{TBA}}
 \begin{algorithmic}[1]
 \label{alg:episode_selection}
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \REQUIRE $startUpdated$, $rewardDiff$, $rewardThresh$
 \ENSURE $episodeVector$
 \IF {($currEpisode == 0$)}
    \STATE $episode$ = [0, 0]
 \ELSIF{($startUpdated$)} 
    \STATE $episodeVector[1]$ += 1
 \ELSE
    \IF{($rewardDiff[0] > rewardThresh$)}
        \STATE $episodeVector[0]$ += 1  
    \ELSIF {($rewardDiff[1] > rewardThresh$)}
        \STATE $episodeVector[1]$ += 1  
    \ELSE
        $episodeVector[0]$ += 1
        $episodeVector[1]$ += 1
    \ENDIF
\ENDIF

\RETURN $episodeVector$
\end{algorithmic}
\end{algorithm}


==> bib.tex <==
\begin{thebibliography}{99}

\bibitem{c1}C. E. Rasmussen and C. K. I. Williams, "Gaussian processes for machine
learning". MA, USA: MIT Press, 2006.
\bibitem{c2}E. Brochu, V. M. Cora, and N. De Freitas, “A tutorial on Bayesian optimization of expensive cost functions, with application to active user modeling and hierarchical reinforcement learning,” 2010, arXiv:1012.2599.
\bibitem{Keyframe-based_Learning_from_Demonstrations}B. Akgun, M. Cakmak, K. Jiang, A. L. Thomaz, "Keyframe-based Learning from Demonstration," Int J of Soc Robotics 4, 343–355 2012. 
\bibitem{c4}L. R. Rabiner, "A tutorial on hidden Markov models and selected applications in speech recognition," in Proceedings of the IEEE, vol. 77, no. 2, pp. 257-286, Feb. 1989, doi: 10.1109/5.18626.
\bibitem{reward_learning_from_very_few_demonstrations}C. Eteke, D. Kebüde and B. Akgün, "Reward Learning From Very Few Demonstrations," in IEEE Transactions on Robotics, vol. 37, no. 3, pp. 893-904, June 2021, doi: 10.1109/TRO.2020.3038698.
\bibitem{robot_learning_from_human_teachers}Sonia C. and  A. L. Thomaz, "Robot Learning from Human Teachers," USA: Morgan & Claypool Publishers, 2014.
\bibitem{simultaneously_learning_actions_and_goals_from_demonstration}B. Akgun and A .Thomaz, "Simultaneously learning actions and goals from demonstration," Auton. Robots 40, 2 (February 2016), 211–227. https://doi.org/10.1007/s10514-015-9448-x
\bibitem{efficient_organized_point_cloud_segmentation_with_connected_components}A. Trevor, S. Gedikli, R. Rusu, and H. Christensen, "Efficient organized point cloud segmentation with connected components," in 3rd Workshop on Semantic Perception Mapping and Exploration (SPME), Karlsruhe, Germany, 2013.
\bibitem{learning_representations_and_generative_models_for_3d_point_clouds} P. Achlioptas, O. Diamanti, I. Mitliagkas, and L. Guibas, "Learning representations and generative models for 3d point clouds," arXiv preprint arXiv:1707.02392, 2017.}
\bibitem{Shapenet:_an_information-rich_3d_model_repository}A. X. Chang, T. Funkhouser, L. Guibas, P. Hanrahan, Q. Huang, Z. Li, S. Savarese, M. Savva, S. Song, H. Su et al., "Shapenet: An information-rich 3d model repository," arXiv preprint arXiv:1512.03012, 2015. Scikit-learn: Machine Learning in Python, Pedregosa et al., JMLR 12, pp. 2825-2830, 2011.
\bibitem{Scikit-learn:_Machine_Learning_in_Python}F. Pedregosa, G. Varoquaux, A. Gramfort, V. Michel, B. Thirion, O. Grisel, M. Blondel, A. Müller, J. Nothman, G. Louppe, P. Prettenhofer, R. Weiss, V. Dubourg, J. Vanderplas, A. Passos, D. Cournapeau, M. Brucher, M. Perrot, and É. Duchesnay, "Scikit-learn: Machine Learning in Python," 2003. [Online]. Available:https://arxiv.org/abs/1201.0490
\bibitem{policy_improvement_methods:between_black-box_optimization_and_episodic_reinforcement_learning}  F. Stulp and O. Sigaud, “Policy improvement: Between black-box optimization and episodic reinforcement learning,” in Proc. Journées Francophones Planification, Décision, et Apprentissage pour la conduite de
systèmes, 2013.
\bibitem{a_survey_on_policy_search_algorithms_for_learning_robot_controllers_in_a_handful_of_trials}K. Chatzilygeroudis, V. Vassiliades, F. Stulp, S. Calinon, and J.-B. Mouret, "A survey on policy search algorithms for learning robot controllers in a handful of trials," IEEE Transactions on Robotics, 2019.
\bibitem{the_cross_entropy_method_for_fast_policy_search}S. Mannor, R. Rubinstein, G. Yohai, "The Cross Entropy method for Fast Policy Search," in Proceedings of the Twentieth International Conference on Machine Learning, 2003 
\bibitem{completely_derandomized_self-adaptation_in_evolution_strategies}N. Hansen and A. Ostermeier, "Completely Derandomized Self-Adaptation in Evolution Strategies," in Evolutionary Computation, vol. 9, no. 2, pp. 159-195, June 2001, doi: 10.1162/106365601750190398.
\bibitem{path_integral_policy_improvement_with_covariance_matrix_adaptation}F. Stulp, O. Sigaud, "Path Integral Policy Improvement with Covariance Matrix Adaptation," in Proceedings of the 10th European Workshop on Reinforcement Learning, 2012 
\bibitem{a_generalized_path_integral_control_approach_to_reinforcement_learning} E. Theodorou, J. Buchli, and S. Schaal, "A generalized path integral control approach to reinforcement learning," journal of machine learning research, vol. 11, no. Nov, pp. 3137–3181, 2010.}
\bibitem{a_tutorial_on_bayesian_optimization_of_expensive_cost_functions_with_application_to_active_user_modeling_and_hierarchical_reinforcement_learning} E. Brochu, V. M. Cora, and N. De Freitas, "A tutorial on Bayesian optimization of expensive cost functions, with application to active user modeling and hierarchical reinforcement learning," 2010, arXiv:1012.2599.}
\bibitem{black-Box_data-efficient_policy_search_for_robotic}K. Chatzilygeroudis, R. Rama, R. Kaushik, D. Goepp, V. Vassiliades, and J.-B. Mouret, "Black-Box Data-efficient Policy Search for Robotics," in IROS, 2017
\bibitem{robots_that_can_adapt_like_animals}A. Cully, J. Clune, D. Tarapore, and J.-B. Mouret, "Robots that can adapt like animals," Nature, vol. 521, no. 7553, pp. 503–507, 2015.
\bibitem{sample_efficient_optimization_for_learning_controllers_for_bipedal_locomotion} R. Antonova, A. Rai, and C. G. Atkeson, "Sample efficient optimization for learning controllers for bipedal locomotion," in Humanoids, 2016.
\bibitem{robot_motor_skill_co-ordination_with_em-based_reinforcement_learning} P. Kormushev, S. Calinon, and D. G. Caldwell, "Robot motor skill co-ordination with em-based reinforcement learning," in Intelligent Robots and Systems (IROS), 2010 IEEE/RSJ International Conference on. IEEE, 2010, pp. 3232–3237.
\bibitem{an_experimental_comparison_of_bayesian_optimization_for_bipedal_locomotion}R. Calandra, A. Seyfarth, J. Peters and M. P. Deisenroth, "An experimental comparison of Bayesian optimization for bipedal locomotion," 2014 IEEE International Conference on Robotics and Automation (ICRA), 2014, pp. 1951-1958, doi: 10.1109/ICRA.2014.6907117.
\bibitem{learning_attractor_landscapes_for_learning_motor_primitives}A. J. Ijspeert, J. Nakanishi, and S. Schaal, "Learning attractor landscapes for learning motor primitives," in Advances in neural information processing systems, 2003, pp. 1547–1554.
\bibitem{conditional_neural_processes} M. Garnelo et al., "Conditional neural processes," Proc. 35th Int. Conf. Mach. Learn., 2018, pp. 1704–1713.

\end{thebibliography}
